Libertas: Privacy-Preserving Collective Computation for Decentralised Personal Data Stores

Data and data processing have become an indispensable aspect for our society. Insights drawn from collective data make invaluable contribution to scientific and societal research and business. But there are increasing worries about privacy issues and data misuse. This has prompted the emergence of decentralised personal data stores (PDS) like Solid that provide individuals more control over their personal data. However, existing PDS frameworks face challenges in ensuring data privacy when performing collective computations with data from multiple users. While Secure Multi-Party Computation (MPC) offers input secrecy protection during the computation without relying on any single party, issues emerge when directly applying MPC in the context of PDS, particularly due to key factors like autonomy and decentralisation. In this work, we discuss the essence of this issue, identify a potential solution, and introduce a modular architecture, Libertas, to integrate MPC with PDS like Solid, without requiring protocol-level changes. We introduce a paradigm shift from an `omniscient' view to individual-based, user-centric view of trust and security, and discuss the threat model of Libertas. Two realistic use cases for collaborative data processing are used for evaluation, both for technical feasibility and empirical benchmark, highlighting its effectiveness in empowering gig workers and generating differentially private synthetic data. The results of our experiments underscore Libertas' linear scalability and provide valuable insights into compute optimisations, thereby advancing the state-of-the-art in privacy-preserving data processing practices. By offering practical solutions for maintaining both individual autonomy and privacy in collaborative data processing environments, Libertas contributes significantly to the ongoing discourse on privacy protection in data-driven decision-making contexts.

==> 1-Intro-bak.tex <==
\section{Introduction}

Data is a valuable resource for science and business, and also for the society and individuals. There is a growing imperative to leverage collective information for societal benefit. Examples include enhancing pandemic responses by aggregating health records~\cite{troncoso_decentralized_2020}, addressing climate change through energy consumption data exchange~\cite{baeck_using_2020}, and even ameliorating working conditions by pooling telemetry data among otherwise isolated gig workers \cite{zhang_algorithmic_2022,stein_you_2023}.

Previous CSCW work has extensively discussed the benefits of user-centric or user-led approaches of collaboration to extract collective insights \cite{calacci_bargaining_2022,lam_enduser_2022,gupta_instagram_2022,zieglmeier_rethinking_2023}, also arguing about the necessity of data autonomy. However, most often, they still make use of a trusted central party (the system) possessing or having direct access to data, and also performing the computation. Architecturally, this exhibits a similar pattern to the platform-led centralised services, and would raise concerns of the same issue of centralised platforms nowadays \cite{tandon_hostile_2022}. Ideally, in a truly user-centric design, the necessity of such a central party should be eliminated, thus addressing the cold-start and trust-obtaining issues.


In the meantime, in recent years, the general public is gaining more attention to the issues of centralised platforms \cite{2021konradgdpr,zuboff2019age}.
Personal Data Stores (PDS) \cite{2014openpds,2016databox,2016solid} are deemed as a promising decentralised approach for addressing the privacy and autonomy concerns for individuals, as they promote a paradigm shift from platform-centred architectures to user-centric architectures. They allow individuals to store their data into a place they trust, and decide (authorise) what applications or services are allowed to use (which part of) their data. This aligns well with the autonomy and user-centric aspects for the collaborative computation, and can form the foundation for the technical realisation.
However, despite the promise in individual-based tasks, collaborative computation is a challenge when privacy-preservation is taken into account (see Sec \ref{sec:background:pds}).

In contrast, algorithmic mechanisms provide technical solutions to enhance privacy (confidentiality) of data use. For example, Secure Multi-Party Computation (MPC) \cite{yao_protocols_1982,lindell_secure_2020} enables the secure evaluation of functions over multiple parties' data without revealing inputs; Differential Privacy (DP) \cite{dwork_differential_2008} aims to mitigate concerns regarding inferring input from computation outputs. However, their discussion mainly focuses on the theoretical benefits, and, as we will see later (Sec \ref{sec:background_privacy} and Sec \ref{sec:mpc-challenges-with-pds}), challenges exist in a user-autonomous setting.


This paper seeks to answer a natural yet under-explored question: is it feasible to perform collaborative computation in a decentralised context while respecting key value expectations?
As minimum core requirements, the solution should address five requirements (also summarised in Table \ref{tab:req_ppc}): for societal value concerns, can the technology support users' data autonomy, address data privacy\footnote{In most computer-science literature, especially privacy-preserving computation, \emph{confidentiality} is the key focus of privacy. For convenience, we keep this convention, and refer the \emph{control} aspect as \emph{autonomy}.} concerns, without imposing a significant trust requirement/assumption; for functional considerations, can the technology scale with the large amount of stakeholders, especially data providers, and support any type of computation?

\begin{table*}
    \centering
    \caption{Crucial functional requirements for a collective privacy-preserving computation system in decentralised context without a central trusted party.}
    \label{tab:req_ppc}
    \begin{tabular}{ll}
        \toprule
        \textbf{Requirement} & \textbf{Explanation} \\
        \midrule
        R1: Privacy & Keeps input data private during computation; \\
        % R1: Privacy & \begin{tabular}{@{}l@{}} Keeps input data private during computation;\\ Optionally, protect the output of the computation from being used to infer the input.\end{tabular} \\
        % \hline
        R2: Autonomy & Gives meaningful control to the data providers/owners over permitted usage of their data.\\
        % \hline
        R3: Minimum Trust & Requires minimum and well-reasoned trust assumptions. \\
        % \hline
        % \item Decentralisation: Data providers have diverse preferences on the trusted parties;
        R4: Scalability & Scales well with the number of data providers. \\
        % \hline
        R5: Generality & Supports all types of computation. \\
        \bottomrule
    \end{tabular}
\end{table*}


In the remaining part of this paper, we identify the shortcomings of current practices (Sec \ref{sec:background}) and the challenges in combining MPC with PDS (Sec \ref{sec:mpc-challenges-with-pds}). These challenges stem from the Autonomy (R2) and Minimum Trust (R3) requirements and the involvement of numerous autonomous data providers not typically encountered in centralised settings. We introduce Libertas (Sec \ref{sec:solid_mpc}), a pioneering modular architecture that addresses \emph{how} to combine MPC with PDS to support collective privacy-preserving computation in decentralised contexts, without requiring changes to underlying protocols. We demonstrate our implementation based on Solid, and discuss its adaptability to other PDS systems.
The proposed architecture utilises the delegated-decentralised MPC model, offering superior scalability (linearly with the number of data providers) compared to the direct-decentralised model, as validated through benchmarking (Sec \ref{sec:benchmark:mpc-models}). We discuss the implications of user-centric trust and the threat model of Libertas (Sec \ref{sec:solid_mpc:threats}). We further evaluate the Libertas architecture with realistic use cases (Sec \ref{sec:evaluation:solid-mpc}), including gig worker empowerment and synthetic differentially-private data generation. These evaluations confirm the technical feasibility and scalability of our approach, showcasing its broad applicability and potential.



\paragraph*{Contributions:} This paper makes both theoretical and practical contributions, as summarised below:
\begin{enumerate}
    \item It highlights a distinct challenge and gap in employing Multi-Party Computation (MPC) in decentralised user-autonomous contexts such as Personal Data Stores (PDS);
    \item It proposes a technical solution, Libertas, to address the issues, as well as highlights the necessity and implications of user-centric trust, in contrast to the omniscience trust in existing literature;
    \item Through two case studies of individual-based collaborative computation, gig worker empowerment and synthetic data generation, it empirically evaluates the proposed system:
    \begin{itemize}
        \item Theoretically, they demonstrate how Libertas can contribute to CSCW for achieving collective benefits \textbf{and} strengthening individual privacy and autonomy simultaneously; the discussion also reveals how real-life power dynamics can achieve the required trust relationships in Libertas to foster adoption;
        \item Practically, they validate the implementation, demonstrate scalability patterns, and identify practical insights.
    \end{itemize}
\end{enumerate}


==> reviewing.tex <==
% Packages
\usepackage[normalem]{ulem} % wavy underlines
\usepackage{xcolor}

% Comments
\newcommand{\todo}[1]{\noindent\textcolor{red}{{\bf \{TODO}: #1{\bf \}}}}
\newcommand{\TODO}[1]{\todo{#1}}
\newcommand{\citeneeded}{\textcolor{red}{{\bf [?!]}}}
\newenvironment{draft}{\color{gray}}{\color{black}}

% Reviewers
\newcommand\rv[1]{{\color{RubineRed}\textbf{RV}: #1}}

\newcommand\rz[1]{{\color{blue}\textbf{RZ}: #1}}

% Annotations
\makeatletter
\font\uwavefont=lasyb10 scaled 700
\def\spelling{\bgroup\markoverwith{\lower3.5\p@\hbox{\uwavefont\textcolor{Red}{\char58}}}\ULon}
\def\grammar{\bgroup\markoverwith{\lower3.5\p@\hbox{\uwavefont\textcolor{LimeGreen}{\char58}}}\ULon}
\def\phrasing{\bgroup\markoverwith{\lower3.5\p@\hbox{\uwavefont\textcolor{RoyalBlue}{\char58}}}\ULon}
\let\rephrase\phrasing
\newcommand\remove{\bgroup\markoverwith{\textcolor{red}{\rule[0.5ex]{2pt}{0.4pt}}}\ULon}
\makeatother

